L2G2G: a Scalable Local-to-Global Network Embedding with Graph Autoencoders

For analysing real-world networks, graph representation learning is a popular tool. These methods, such as a graph autoencoder (GAE), typically rely on low-dimensional representations, also called embeddings, which are obtained through minimising a loss function; these embeddings are used with a decoder for downstream tasks such as node classification and edge prediction. While GAEs tend to be fairly accurate, they suffer from scalability issues. For improved speed, a Local2Global approach, which combines graph patch embeddings based on eigenvector synchronisation, was shown to be fast and achieve good accuracy. Here we propose L2G2G, a Local2Global method which improves GAE accuracy without sacrificing scalability. This improvement is achieved by dynamically synchronising the latent node representations, while training the GAEs. It also benefits from the decoder computing an only local patch loss. Hence, aligning the local embeddings in each epoch utilises more information from the graph than a single post-training alignment does, while maintaining scalability. We illustrate on synthetic benchmarks, as well as real-world examples, that L2G2G achieves higher accuracy than the standard Local2Global approach and scales efficiently on the larger data sets. We find that for large and dense networks, it even outperforms the slow, but assumed more accurate, GAEs.

==> oldbib.tex <==
@article{local2global,
  title={Local2Global: Scaling global representation learning on graphs via local training},
  author={Jeub, Lucas GS and Colavizza, Giovanni and Dong, Xiaowen and Bazzi, Marya and Cucuringu, Mihai},
  journal={arXiv preprint arXiv:2107.12224},
  year={2021}
}


@article{vgae,
  title={Variational graph auto-encoders},
  author={Kipf, Thomas N and Welling, Max},
  journal={arXiv preprint arXiv:1611.07308},
  year={2016}
}

@article{fastgae,
  title={FastGAE: Scalable graph autoencoders with stochastic subgraph decoding},
  author={Salha, Guillaume and Hennequin, Romain and Remy, Jean-Baptiste and Moussallam, Manuel and Vazirgiannis, Michalis},
  journal={Neural Networks},
  volume={142},
  pages={1--19},
  year={2021},
  publisher={Elsevier}
}


@article{scalable-gnn-via-bp,
  author    = {Ming Chen and
               Zhewei Wei and
               Bolin Ding and
               Yaliang Li and
               Ye Yuan and
               Xiaoyong Du and
               Ji{-}Rong Wen},
  title     = {Scalable Graph Neural Networks via Bidirectional Propagation},
  journal   = {CoRR},
  volume    = {abs/2010.15421},
  year      = {2020},
  url       = {https://arxiv.org/abs/2010.15421},
  eprinttype = {arXiv},
  eprint    = {2010.15421},
  timestamp = {Tue, 03 Nov 2020 11:44:23 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2010-15421.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@article{sc,
author = {Tang, Lei and Liu, Huan},
title = {Leveraging Social Media Networks for Classification},
year = {2011},
issue_date = {November 2011},
publisher = {Kluwer Academic Publishers},
address = {USA},
volume = {23},
number = {3},
issn = {1384-5810},
url = {https://doi.org/10.1007/s10618-010-0210-x},
doi = {10.1007/s10618-010-0210-x},
abstract = {Social media has reshaped the way in which people interact with each other. The rapid development of participatory web and social networking sites like YouTube, Twitter, and Facebook, also brings about many data mining opportunities and novel challenges. In particular, we focus on classification tasks with user interaction information in a social network. Networks in social media are heterogeneous, consisting of various relations. Since the relation-type information may not be available in social media, most existing approaches treat these inhomogeneous connections homogeneously, leading to an unsatisfactory classification performance. In order to handle the network heterogeneity, we propose the concept of social dimension to represent actors' latent affiliations, and develop a classification framework based on that. The proposed framework, SocioDim, first extracts social dimensions based on the network structure to accurately capture prominent interaction patterns between actors, then learns a discriminative classifier to select relevant social dimensions. SocioDim, by differentiating different types of network connections, outperforms existing representative methods of classification in social media, and offers a simple yet effective approach to integrating two types of seemingly orthogonal information: the network of actors and their attributes.},
journal = {Data Min. Knowl. Discov.},
month = {nov},
pages = {447–478},
numpages = {32},
keywords = {Collective inference, Social media, Social network analysis, Within-network classification, Relational learning}
}

@inproceedings{dw,
	doi = {10.1145/2623330.2623732},
  
	url = {https://doi.org/10.1145%2F2623330.2623732},
  
	year = 2014,
	month = {aug},
  
	publisher = {{ACM}
},
  
	author = {Bryan Perozzi and Rami Al-Rfou and Steven Skiena},
  
	title = {{DeepWalk}},
  
	booktitle = {Proceedings of the 20th {ACM} {SIGKDD} international conference on Knowledge discovery and data mining}
}

@inproceedings{graphsaint,
title={GraphSAINT: Graph Sampling Based Inductive Learning Method},
author={Hanqing Zeng and Hongkuan Zhou and Ajitesh Srivastava and Rajgopal Kannan and Viktor Prasanna},
booktitle={International Conference on Learning Representations},
year={2020},
url={https://openreview.net/forum?id=BJe8pkHFwS}
}


@misc{graphsage,
  doi = {10.48550/ARXIV.1706.02216},
  
  url = {https://arxiv.org/abs/1706.02216},
  
  author = {Hamilton, William L. and Ying, Rex and Leskovec, Jure},
  
  keywords = {Social and Information Networks (cs.SI), Machine Learning (cs.LG), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Inductive Representation Learning on Large Graphs},
  
  publisher = {arXiv},
  
  year = {2017},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{fastgcn,
  doi = {10.48550/ARXIV.1801.10247},
  
  url = {https://arxiv.org/abs/1801.10247},
  
  author = {Chen, Jie and Ma, Tengfei and Xiao, Cao},
  
  keywords = {Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {FastGCN: Fast Learning with Graph Convolutional Networks via Importance Sampling},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{hamilton2017inductive,
  title={Inductive representation learning on large graphs},
  author={Hamilton, Will and Ying, Zhitao and Leskovec, Jure},
  journal={Advances in Neural Information Processing Systems},
  volume={30},
  year={2017}
}


@article{he2021fedgraphnn,
  publtype={informal},
  author={Chaoyang He and Keshav Balasubramanian and Emir Ceyani and Yu Rong and Peilin Zhao and Junzhou Huang and Murali Annavaram and Salman Avestimehr},
  title={FedGraphNN: A Federated Learning System and Benchmark for Graph Neural Networks},
  year={2021},
  cdate={1609459200000},
  journal={CoRR},
  volume={abs/2104.07145},
  url={https://arxiv.org/abs/2104.07145}
}


@misc{sgc,
  doi = {10.48550/ARXIV.2007.02133},
  
  url = {https://arxiv.org/abs/2007.02133},
  
  author = {Chen, Ming and Wei, Zhewei and Huang, Zengfeng and Ding, Bolin and Li, Yaliang},
  
  keywords = {Machine Learning (cs.LG), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Simple and Deep Graph Convolutional Networks},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{pprgo,
	doi = {10.1145/3394486.3403296},
  
	url = {https://doi.org/10.1145%2F3394486.3403296},
  
	year = 2020,
	month = {aug},
  
	publisher = {{ACM}
},
  
	author = {Aleksandar Bojchevski and Johannes Klicpera and Bryan Perozzi and Amol Kapoor and Martin Blais and Benedek R{\'{o}}zemberczki and Michal Lukasik and Stephan Günnemann},
  
	title = {Scaling Graph Neural Networks with Approximate {PageRank}},
  
	booktitle = {Proceedings of the 26th {ACM} {SIGKDD} International Conference on Knowledge Discovery \&  Data Mining}
}

@inproceedings{cluster-gcn,
	doi = {10.1145/3292500.3330925},
  
	url = {https://doi.org/10.1145%2F3292500.3330925},
  
	year = 2019,
	month = {jul},
  
	publisher = {{ACM}
},
  
	author = {Wei-Lin Chiang and Xuanqing Liu and Si Si and Yang Li and Samy Bengio and Cho-Jui Hsieh},
  
	title = {Cluster-{GCN}},
  
	booktitle = {Proceedings of the 25th {ACM} {SIGKDD} International Conference on Knowledge Discovery \& Data Mining}
}

@article{es1,
author = {Cucuringu, Mihai and Lipman, Yaron and Singer, Amit},
title = {Sensor Network Localization by Eigenvector Synchronization over the Euclidean Group},
year = {2012},
issue_date = {July 2012},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {8},
number = {3},
issn = {1550-4859},
url = {https://doi.org/10.1145/2240092.2240093},
doi = {10.1145/2240092.2240093},
abstract = {We present a new approach to localization of sensors from noisy measurements of a subset of their Euclidean distances. Our algorithm starts by finding, embedding, and aligning uniquely realizable subsets of neighboring sensors called patches. In the noise-free case, each patch agrees with its global positioning up to an unknown rigid motion of translation, rotation, and possibly reflection. The reflections and rotations are estimated using the recently developed eigenvector synchronization algorithm, while the translations are estimated by solving an overdetermined linear system. The algorithm is scalable as the number of nodes increases and can be implemented in a distributed fashion. Extensive numerical experiments show that it compares favorably to other existing algorithms in terms of robustness to noise, sparse connectivity, and running time. While our approach is applicable to higher dimensions, in the current article, we focus on the two-dimensional case.},
journal = {ACM Trans. Sen. Netw.},
month = {aug},
articleno = {19},
numpages = {42},
keywords = {synchronization, spectral graph theory, rigidity theory, Sensor networks, eigenvectors, distance geometry}
}

@article{es2,
	doi = {10.1093/imaiai/ias002},
  
	url = {https://doi.org/10.1093%2Fimaiai%2Fias002},
  
	year = 2012,
	month = {dec},
  
	publisher = {Oxford University Press ({OUP})},
  
	volume = {1},
  
	number = {1},
  
	pages = {21--67},
  
	author = {M. Cucuringu and A. Singer and D. Cowburn},
  
	title = {Eigenvector synchronization, graph rigidity and the molecule problem},
  
	journal = {Information and Inference}
}
@inproceedings{Cora&ML,
title={Deep Gaussian Embedding of Graphs:  Unsupervised Inductive Learning via Ranking},
author={Aleksandar Bojchevski and Stephan Günnemann},
booktitle={International Conference on Learning Representations},
year={2018},
url={https://openreview.net/forum?id=r1ZdKJ-0W},
}

@article{bruna2013spectral,
  title={Spectral networks and locally connected networks on graphs},
  author={Bruna, Joan and Zaremba, Wojciech and Szlam, Arthur and LeCun, Yann},
  journal={arXiv preprint arXiv:1312.6203},
  year={2013}
}

@misc{gnn,
  doi = {10.48550/ARXIV.1312.6203},
  
  url = {https://arxiv.org/abs/1312.6203},
  
  author = {Bruna, Joan and Zaremba, Wojciech and Szlam, Arthur and LeCun, Yann},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), Neural and Evolutionary Computing (cs.NE), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Spectral Networks and Locally Connected Networks on Graphs},
  
  publisher = {arXiv},
  
  year = {2013},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{chen2020simple,
  title={Simple and deep graph convolutional networks},
  author={Chen, Ming and Wei, Zhewei and Huang, Zengfeng and Ding, Bolin and Li, Yaliang},
  booktitle={International Conference on Machine Learning},
  pages={1725--1735},
  year={2020},
  organization={PMLR}
}

@article{chen2020scalable,
  title={Scalable graph neural networks via bidirectional propagation},
  author={Chen, Ming and Wei, Zhewei and Ding, Bolin and Li, Yaliang and Yuan, Ye and Du, Xiaoyong and Wen, Ji-Rong},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={14556--14566},
  year={2020}
}

@article{chen2018fastgcn,
  title={Fastgcn: fast learning with graph convolutional networks via importance sampling},
  author={Chen, Jie and Ma, Tengfei and Xiao, Cao},
  journal={arXiv preprint arXiv:1801.10247},
  year={2018}
}


@article{FL+GNN1,
  title={FedWalk: Communication Efficient Federated Unsupervised Node Embedding with Differential Privacy},
  author={Pan, Qiying and Zhu, Yifei},
  journal={arXiv preprint arXiv:2205.15896},
  year={2022}
}

@misc{FL+GNN2,
  doi = {10.48550/ARXIV.2104.07145},
  
  url = {https://arxiv.org/abs/2104.07145},
  
  author = {He, Chaoyang and Balasubramanian, Keshav and Ceyani, Emir and Yang, Carl and Xie, Han and Sun, Lichao and He, Lifang and Yang, Liangwei and Yu, Philip S. and Rong, Yu and Zhao, Peilin and Huang, Junzhou and Annavaram, Murali and Avestimehr, Salman},
  
  keywords = {Machine Learning (cs.LG), Artificial Intelligence (cs.AI), Distributed, Parallel, and Cluster Computing (cs.DC), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {FedGraphNN: A Federated Learning System and Benchmark for Graph Neural Networks},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {Creative Commons Attribution 4.0 International}
}
@INPROCEEDINGS{FL+GNN3,
  author={Mei, Guangxu and Guo, Ziyu and Liu, Shijun and Pan, Li},
  booktitle={2019 IEEE International Conference on Big Data (Big Data)}, 
  title={SGNN: A Graph Neural Network Based Federated Learning Approach by Hiding Structure}, 
  year={2019},
  volume={},
  number={},
  pages={2560-2568},
  doi={10.1109/BigData47090.2019.9005983}}


@article{Graph-clustering-with-GNN,
  title={Graph clustering with graph neural networks},
  author={Tsitsulin, Anton and Palowitch, John and Perozzi, Bryan and M{\"u}ller, Emmanuel},
  journal={arXiv preprint arXiv:2006.16904},
  year={2020}
}


@InProceedings{Spectral-clustering-with-GNN,
  title = 	 {Spectral Clustering with Graph Neural Networks for Graph Pooling},
  author =       {Bianchi, Filippo Maria and Grattarola, Daniele and Alippi, Cesare},
  booktitle = 	 {Proceedings of the 37th International Conference on Machine Learning},
  pages = 	 {874--883},
  year = 	 {2020},
  editor = 	 {III, Hal Daumé and Singh, Aarti},
  volume = 	 {119},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {13--18 Jul},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v119/bianchi20a/bianchi20a.pdf},
  url = 	 {https://proceedings.mlr.press/v119/bianchi20a.html},
  abstract = 	 {Spectral clustering (SC) is a popular clustering technique to find strongly connected communities on a graph. SC can be used in Graph Neural Networks (GNNs) to implement pooling operations that aggregate nodes belonging to the same cluster. However, the eigendecomposition of the Laplacian is expensive and, since clustering results are graph-specific, pooling methods based on SC must perform a new optimization for each new sample. In this paper, we propose a graph clustering approach that addresses these limitations of SC. We formulate a continuous relaxation of the normalized minCUT problem and train a GNN to compute cluster assignments that minimize this objective. Our GNN-based implementation is differentiable, does not require to compute the spectral decomposition, and learns a clustering function that can be quickly evaluated on out-of-sample graphs. From the proposed clustering method, we design a graph pooling operator that overcomes some important limitations of state-of-the-art graph pooling techniques and achieves the best performance in several supervised and unsupervised tasks.}
}

@inproceedings{bayer2022label,
  title={Label Propagation Across Graphs: Node Classification Using Graph Neural Tangent Kernels},
  author={Bayer, Artun and Chowdhury, Arindam and Segarra, Santiago},
  booktitle={ICASSP 2022-2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={5483--5487},
  year={2022},
  organization={IEEE}
}

@misc{Node-classification-with-Graph-Tangent-kernal,
  doi = {10.48550/ARXIV.2110.03763},
  
  url = {https://arxiv.org/abs/2110.03763},
  
  author = {Bayer, Artun and Chowdhury, Arindam and Segarra, Santiago},
  
  keywords = {Machine Learning (cs.LG), Signal Processing (eess.SP), FOS: Computer and information sciences, FOS: Computer and information sciences, FOS: Electrical engineering, electronic engineering, information engineering, FOS: Electrical engineering, electronic engineering, information engineering},
  
  title = {Label Propagation across Graphs: Node Classification using Graph Neural Tangent Kernels},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{node-classification-gnn2,
  title={Bag of tricks for node classification with graph neural networks},
  author={Wang, Yangkun and Jin, Jiarui and Zhang, Weinan and Yu, Yong and Zhang, Zheng and Wipf, David},
  journal={arXiv preprint arXiv:2103.13355},
  year={2021}
}


@article{link-prediction-on-gnn,
  title={Link prediction based on graph neural networks},
  author={Zhang, Muhan and Chen, Yixin},
  journal={Advances in Neural Information Processing Systems},
  volume={31},
  year={2018}
}


@inproceedings{
link-prediction-gnn2,
title={Labeling Trick: A Theory of Using Graph Neural Networks for Multi-Node Representation Learning},
author={Muhan Zhang and Pan Li and Yinglong Xia and Kai Wang and Long Jin},
booktitle={Advances in Neural Information Processing Systems},
editor={A. Beygelzimer and Y. Dauphin and P. Liang and J. Wortman Vaughan},
year={2021},
url={https://openreview.net/forum?id=Hcr9mgBG6ds}
}


@inproceedings{adam,
  author={Diederik P. Kingma and Jimmy Ba},
  title={Adam: A Method for Stochastic Optimization},
  year={2015},
  cdate={1420070400000},
  url={http://arxiv.org/abs/1412.6980},
  booktitle={ICLR (Poster)},
  crossref={conf/iclr/2015}
}

@article{SBM,
	doi = {10.1103/physreve.83.016107},
  
	url = {https://doi.org/10.1103%2Fphysreve.83.016107},
  
	year = 2011,
	month = {jan},
  
	publisher = {American Physical Society ({APS})},
  
	volume = {83},
  
	number = {1},
  
	author = {Brian Karrer and M. E. J. Newman},
  
	title = {Stochastic blockmodels and community structure in networks},
  
	journal = {Physical Review E}
}

@article{gcn,
  title={Graph convolutional networks: a comprehensive review},
  author={Zhang, Si and Tong, Hanghang and Xu, Jiejun and Maciejewski, Ross},
  journal={Computational Social Networks},
  volume={6},
  number={1},
  pages={1--23},
  year={2019},
  publisher={SpringerOpen}
}


@misc{local2,
	author = {Jeub, Lucas G. S.},
	date-added = {2022-08-15 19:07:24 +0100},
	date-modified = {2022-08-15 19:09:42 +0100},
	howpublished = {Github \url{https://github.com/LJeub/Local2Global}},
	month = {August},
	title = {Local2Global Github package},
	year = {2021}}


@software{pytorchGeo,
author = {Fey, Matthias and Lenssen, Jan Eric},
license = {MIT},
month = {5},
title = {{Fast Graph Representation Learning with PyTorch Geometric}},
url = {https://github.com/pyg-team/pytorch_geometric},
year = {2019}
}

@inproceedings{su2015relationship,
  title={A relationship between the average precision and the area under the ROC curve},
  author={Su, Wanhua and Yuan, Yan and Zhu, Mu},
  booktitle={Proceedings of the 2015 International Conference on The Theory of Information Retrieval},
  pages={349--352},
  year={2015}
}

@article{LADIES,
  title={Layer-dependent importance sampling for training deep and large graph convolutional networks},
  author={Zou, Difan and Hu, Ziniu and Wang, Yewen and Jiang, Song and Sun, Yizhou and Gu, Quanquan},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}


